Towards an Ontology-Driven Approach for Process-Aware Risk Propagation

The rapid development of cyber-physical systems creates an increasing demand for a general approach to risk, especially considering how physical and digital components affect the processes of the system itself. In risk analytics and management, risk propagation is a central technique, which allows the calculation of the cascading effect of risk within a system and supports risk mitigation activities. However, one open challenge is to devise a process-aware risk propagation solution that can be used to assess the impact of risk at different levels of abstraction, accounting for actors, processes, physical-digital objects, and their interrelations. To address this challenge, we propose a process-aware risk propagation approach that builds on two main components: i. an ontology, which supports functionalities typical of Semantic Web technologies (SWT), and semantics-based intelligent systems, representing a system with processes and objects having different levels of abstraction, and ii. a method to calculate the propagation of risk within the given system. We implemented our approach in a proof-of-concept tool, which was validated and demonstrated in the cybersecurity domain.

==> authors.tex <==
\author{Gal Engelberg}
%\authornote{Dr.~Trovato insisted his name be first.}
%\orcid{1234-5678-9012}
\affiliation{%
  \institution{Accenture Labs, University of Haifa}
  \streetaddress{P.O. Box 1212}
  \city{Haifa} 
  \country{Israel} 
  %\postcode{43017-6221}
}
\email{gal.engelberg@accenture.com}
%ORCID - 0000-0001-9021-9740

\author{Mattia Fumagalli}
%\authornote{The secretary disavows any knowledge of this author's actions.}
\affiliation{%
  \institution{Free University of Bozen-Bolzano}
  %\streetaddress{P.O. Box 1212}
  \city{Bolzano} 
  \country{Italy} 
  %\postcode{43017-6221}
}
\email{mattia.fumagalli@unibz.it}

\author{Adrian Kuboszek}
%\authornote{This author is the
%  one who did all the really hard work.}
\affiliation{%
  \institution{Avanade}
  %\streetaddress{1 Th{\o}rv{\"a}ld Circle}
  %\city{Hekla} 
  \country{Poland}}
\email{a.kuboszek@avanade.com}

%ORCID - 0000-0002-9493-1476

\author{Dan Klein}
\affiliation{%
  \institution{Accenture Labs}
  %\city{Rocquencourt}
  \country{Israel}}
  \email{dan.klein@accenture.com}

%https://orcid.org/0000-0002-8881-1902

\author{Pnina Soffer} 
\affiliation{%
 \institution{University of Haifa}
 %\streetaddress{Rono-Hills}
 \city{Haifa} 
 %\state{Arunachal Pradesh}
 \country{Israel}}
\email{spnina@is.haifa.ac.il}
%ORCID - 0000-0003-4659-883X
 
\author{Giancarlo Guizzardi}
\affiliation{%
  \institution{University of Twente}
  %\streetaddress{30 Shuangqing Rd}
  %\city{Haidian Qu} 
  %\state{Beijing Shi}
  \country{The Netherlands}
}
\email{g.guizzardi@utwente.nl}
%ORCID - 0000-0002-3452-553X
